Influence Maximization Based on Dynamic Personal Perception in Knowledge Graph

Viral marketing on social networks, also known as Influence Maximization (IM), aims to select k users for the promotion of a target item by maximizing the total spread of their influence. However, most previous works on IM do not explore the dynamic user perception of promoted items in the process. In this paper, by exploiting the knowledge graph (KG) to capture dynamic user perception, we formulate the problem of Influence Maximization with Dynamic Personal Perception (IMDPP) that considers user preferences and social influence reflecting the impact of relevant item adoptions. We prove the hardness of IMDPP and design an approximation algorithm, named Dynamic perception for seeding in target markets (Dysim), by exploring the concepts of dynamic reachability, target markets, and substantial influence to select and promote a sequence of relevant items. We evaluate the performance of Dysim in comparison with the state-of-the-art approaches using real social networks with real KGs. The experimental results show that Dysim effectively achieves up to 6.7 times of influence spread in large datasets over the state-of-the-art approaches.

==> Fig/fig_ex.tex <==
\begin{figure}[t]
\centering
\subfigure[][A knowledge graph.]{
\centering
\label{Fig:ex_kg}
\begin{tikzpicture}
    \node[item node] (iphone) {iPhone 11};
    \node[company node] (apple) [above right = 0.7cm and 1.55cm of iphone] {Apple};
    \node[event node] (selfie) [below = 0.7cm of iphone] {selfie};
    \node[item node] (charging_cable) [above = 0.5cm of iphone] {charging\\cable};
    \node[item node] (airpods) [right = 1.4cm of iphone] {AirPods};
    \node[item node] (selfie_stick) [below right = 0.51cm and 1.5cm of iphone] {selfie\\stick};

	\path[edge] (apple) edge [bend left=10] node [below,pos=0.3] {has} (iphone);
	\path[edge] (apple) edge node {has} (charging_cable);
	\path[edge] (apple) edge node [swap] {has} (airpods);
	\path[edge] (airpods) edge node {supports} (iphone);
	\path[edge] (iphone) edge node [swap] {relies on} (charging_cable);
	\path[edge] (selfie) edge node [swap,pos=0.3] {needs} (iphone);
	\path[edge] (selfie) edge node [swap] {needs} (selfie_stick);
	\path[edge] (selfie_stick) edge [bend left=10] node [swap] {supports} (iphone);
\end{tikzpicture}
}%
\subfigure[][Meta-graphs for the complementary relationship.]{
\centering
\label{Fig:ex_meta}
\begin{tikzpicture}
	\node[fill=none,draw=none,font=\small] (m1) {$m^c_1$: };
	\node[item node, font=\scshape\small] (i1) [below right = 0cm and 0.1cm of m1] {item};
	\node[item node, font=\scshape\small] [right = 1.5cm of i1] (i2) {item};
	\node[company node, font=\scshape\small] (c) [above right = 0.5cm and 0.05cm of i1] {company};
	\node[fill=none,draw=none,font=\small] (m2) [below = 1cm of m1] {$m^c_2$: };
	\node[item node, font=\scshape\small] (i3) [below right = 0cm and 0.1cm of m2] {item};
	\node[item node, font=\scshape\small] [right = 1.5cm of i3] (i4) {item};
	\node[event node, font=\scshape\small] (e) [above right = 0.5cm and 0.55cm of i3] {event};

	\path[edge] (i1) edge node {relies on} (i2);
	\path[edge] (c) edge node [swap,pos=0.6] {has} (i1);
	\path[edge] (c) edge node [pos=0.6] {has} (i2);
	\path[edge] (i4) edge node {supports} (i3);
	\path[edge] (e) edge node [swap,pos=0.7] {needs} (i3);
	\path[edge] (e) edge node [pos=0.6] {needs} (i4);
\end{tikzpicture}
}
\hfill
\caption{An illustrating example.}
\label{Fig:ex}
\end{figure}
